Language Model Evaluation in Open-ended Text Generation

Although current state-of-the-art language models have achieved impressive results in numerous natural language processing tasks, still they could not solve the problem of producing repetitive, dull and sometimes inconsistent text in open-ended text generation. Studies often attribute this problem to the maximum likelihood training objective, and propose alternative approaches by using stochastic decoding methods or altering the training objective. However, there is still a lack of consistent evaluation metrics to directly compare the efficacy of these solutions. In this work, we study different evaluation metrics that have been proposed to evaluate quality, diversity and consistency of machine-generated text. From there, we propose a practical pipeline to evaluate language models in open-ended generation task, and research on how to improve the model's performance in all dimensions by leveraging different auxiliary training objectives.

==> Preamble/Abstract.tex <==
\Abstract{

\addtocontents{toc}{\vspace{1em}}  % Add a gap in the Contents, for aesthetics

Although current state-of-the-art language models have achieved impressive results in numerous natural language processing tasks, still they could not solve the problem of producing repetitive, dull and sometimes inconsistent text in open-ended text generation. Studies often attribute this problem to the maximum likelihood training objective, and propose alternative approaches by using stochastic decoding or altering the training objective. One of the promising approaches is unlikelihood training \citep{welleck2019neural, li2019dont}, which not only significantly reduce repetitiveness but also help to produce more consistent text. In this project, we aim to further evaluate unlikelihood training in open-ended text generation using a wide range of evaluation metrics, including language quality, diversity and consistency, compared to other training and decoding methods.

}
